Quantum Random Access Code in Noisy Channels

Random access code (RAC) communication protocol particularly useful when the communication between parties is restricted. In this work we built upon works that have previously proven quantum random access code (QRAC), in the absence of noise, to be more advantageous than classical random access code (CRAC), investigate the effects of noisy channel on QRAC performance and how the losses can be mitigated by using the see-saw method optimized by semi-definite programming when the noisy channel is known.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
